Subquadratic Multivalued Asynchronous Byzantine Agreement WHP

There have been several reductions from multivalued consensus to binary consensus over the past 20 years. To the best of our knowledge, none of them solved it for Byzantine asynchronous settings. In this paper, we close this gap. Moreover, we do so in subquadratic communication, using newly developed subquadratic binary Byzantine Agreement techniques.

==> related_work.tex <==
\section{Related Work}
\label{sec:related_work}


% \paragraph{Lower bounds.}
{\bf Lower bounds.} 
Our assumptions conform with a number of known bounds. Deterministic consensus is impossible in an asynchronous system if even one process may crash (by FLP~\cite{fischer1985impossibility}) and requires $\Omega(n^2)$ communication even in synchronous systems~\cite{DolevBound}. As for randomized Byzantine Agreement, Abraham et al.
\cite{abraham2019communication} state that disallowing
after-the-fact removal is necessary even in synchronous settings for achieving sub-quadratic communication.

% \paragraph{Asynchronous BA and shared coin algorithms.}
{\bf Asynchronous BA and shared coin algorithms.} 
The algorithms we present in this paper belong to the family of asynchronous BA algorithms, which sacrifice determinism in order to circumvent FLP. We compare our solutions to existing ones in Table~\ref{tab:survey}.
 
Ben-Or~\cite{ben1983another} suggested a protocol with resilience $n>5f$. This protocol uses a local coin (namely, a local source of randomness) and its expected time complexity is exponential (or constant if $f=O(\sqrt n)$). Bracha~\cite{bracha1987asynchronous} improved the resilience to $n>3f$ with the same complexity. The complexity can be greatly reduced by replacing the local coin with a shared one with a guaranteed success rate.

Later works presented the shared coin abstraction and used it to solve BA with $O(n^2)$ communication. Rabin~\cite{rabin1983randomized} was the first to do so, suggesting a protocol with resilience $n>10f$ and a constant expected number of rounds. Cachin et al.~\cite{cachin2005random} were the first to use a shared coin to solve BA with $O(n^2)$ communication and optimal resilience.
Mostefaoui et al.~\cite{mostefaoui2015signature} then presented a signature-free BA algorithm with optimal resilience and $O(n^2)$ messages that uses a shared coin abstraction as a black box; the shared coin algorithm we provide in Section 4 can be used to instantiate this protocol. All of the aforementioned algorithms solve binary BA, where the processes’ initial values are 0 and 1; a recent work solved multi-valued BA with the same $O(n^2)$ word complexity~\cite{abraham2019asymptotically}.


BA algorithms also differ in the cryptographic assumptions they make and the cryptographic tools they use. Rabin’s coin~\cite{rabin1983randomized} is based on cryptographic secret sharing~\cite{shamir1979share}. Some later works followed suit, and used cryptographic abstractions such as threshold signatures~\cite{abraham2019asymptotically,cachin2005random}. Other works forgo cryptography altogether and instead consider a full information model, where there are no restrictions on the adversary’s computational power~\cite{canetti1993fast,king2013byzantine}. In this model, the problem is harder, and existing works achieve very low resilience~\cite{king2013byzantine} ($n>400f$) or high communication complexity~\cite{canetti1993fast}. In this paper we do use cryptographic primitives. We assume a computationally bounded adversary and rely on the abstraction of a VRF~\cite{micali1999VRF}. VRFs were previously used in blockchain protocols~\cite{Algorand,hanke2018dfinity,Helix} and were also used by Micali~\cite{DBLP:conf/innovations/Micali17} to construct a shared coin in the synchronous model.


Several works~\cite{Abraham2018HotStuffTL,baudet2019state,kwon2014tendermint,naor2019cogsworth,spiegelman2020search} solve BA with subquadratic complexity in the so-called optimistic case (or ``happy path''), when communication is timely and a correct process is chosen as a ``leader''. In contrast, we focus on the worst-case asynchronous case. 


\begin{table}
\caption{Asynchronous Byzantine Agreement algorithms.}

\setlength\extrarowheight{3pt}

\begin{tabular}{lccccc}

\toprule
% \hline
Protocol & n $>$ & Adversary & Word complexity & Termination & Safety \\

\midrule

Ben-Or~\cite{ben1983another}   & $5f$ & adaptive & $O(2^n)$ & w.p. 1 & $\checkmark$ \\ 


Rabin~\cite{rabin1983randomized}   & $10f$ & adaptive & $O(n^2)$ & w.p. 1 & $\checkmark$ \\ 

Bracha~\cite{bracha1987asynchronous} & $3f$  & adaptive & $O(2^n)$ & w.p. 1 & $\checkmark$ \\ 

Cachin et al.~\cite{cachin2005random} & $3f$  & adaptive & $O(n^2)$ &  w.p. 1 & $\checkmark$ \\ 

King-Saia~\cite{king2013byzantine} & $400f$  & adaptive & polynomial & whp & $\checkmark$ \\ 

MMR~\cite{mostefaoui2015signature} & $3f$  & adaptive & $O(n^2)$ & w.p. 1 & $\checkmark$ \\ 

% Section \ref{sec:shared_coin} + MMR & $\approx3.5f$  & delayed-adaptive & $O(n^2)$ & PKI & w.p. 1 & $\checkmark$ \\ 

Our protocol & $\approx4.5f$  & delayed-adaptive & $\tilde{O}(n)$ & whp & whp \\ 

\bottomrule

\end{tabular}
\label{tab:survey}
\end{table}

% \paragraph{Committees.}
{\bf Committees.} 
We use committees in order to reduce the word complexity and allow each step of the protocol to be executed by only a fraction of the processes. King and Saia used a similar concept and presented the first sub-quadratic BA protocol in the synchronous model~\cite{king2011breaking}. Algorand proposed a synchronous algorithm~\cite{Algorand} (and later extended it to eventual synchrony~\cite{chen2018algorand}) where committees are sampled randomly
using a VRF. Each process executes a local computation to sample itself to a committee, and hence the selection of processes does not require interaction among them. We follow this approach in this paper and adapt the technique to the asynchronous model.
 


Following initial publication of our work, Blum et al.~\cite{cryptoeprint:2020:851} have also achieved subquadratic BA WHP under an adaptive adversary. Their assumptions are incomparable to ours -- while they strengthen the adversary to remove the delayed adaptivity requirement, they also strengthen the trusted setup. Specifically, they use a trusted dealer to a priori determine the committee members, flip the shared coin, and share it among the committee members. In contrast, we use a peer-to-peer protocol to generate randomness, and require delayed adaptivity in order to prevent the adversary from tampering with this randomness. As in our protocol, setup has to occur once and may be used for any number of BA instances.

==> sampling.tex <==



% \subsection{Validated Committee Sampling} 
% \label{sec:committees}


% A common strategy for achieving subquadratic word complexity is to avoid all-to-all communications~\cite{Algorand,king2011breaking}. This is done by sampling subsets of processes such that only those elected to a committee send messages. Due to committees being randomly sampled, the adversary is prevented from corrupting their members. On the other hand, committee members cannot predict the following committee sample and thus send their messages to all processes. Potentially, if the committee is sufficiently small, this technique allows committee-based protocols to result in subquadratic word complexity.

{\bf Validated Committee Sampling.}
Using VRFs, it is possible to implement \emph{validated committee sampling}, which is a primitive that allows processes to elect committees without communication and later prove
their election. It provides every process $p_i$ with a private
function $\emph{sample}_i(s,\lambda)$, which gets a string $s$ and a
threshold $1\leq \lambda \leq n$ and returns a tuple $\lr{v_i,\sigma_i}$, where
$v_i \in \{ \emph{true},\emph{false}\}$ and $\sigma_i$ is a proof that $v_i=\emph{sample}_i(s,\lambda)$. If $v_i=\emph{true}$ we say that $p_i$ is \emph{sampled} to the committee for $s$ and $\lambda$. The primitive ensures that $p_i$ is sampled with probability $\frac{\lambda}{n}$.
In addition, there is a public (known to all) function,
$\emph{committee-val}(s,\lambda,i,\sigma_i)$, which gets a
string $s$, a threshold $\lambda$, a process identification $i$ and a proof
$\sigma_i$, and returns \emph{true} or \emph{false}.



Consider a string $s$.
For every $i$, $1 \leq i \leq n$, let $\lr{v_i,\sigma_i}$ be the return value of $\emph{sample}_i(s,\lambda)$. The following is satisfied for every $p_i$:
%
\begin{itemize}
  
  \item $\emph{committee-val}(s,\lambda,i,\sigma_i) = v_i$.
  
  \item If $p_i$ is correct, then it is infeasible
  for the adversary to compute $\emph{sample}_i(s,\lambda)$.
  
  \item It is infeasible for the adversary to find  $\lr{v, \sigma}$
  s.t.\ $v \neq v_i$ and
  $\emph{committee-val}(s,\lambda,i,\sigma) = true$.
  
\end{itemize}

% In this paper when we use the term whp we mean that the probability of the discussed event is at least $1-\frac{1}{n^c}$ for every constant $c$ and sufficiently large $n$.


% In this work, we take advantage of the validated committee sampling, as defined and used in~\cite{cohen2020not}.
% In their work, Cohen et. al adjusted the use of this primitive to the asynchronous setting. With their technique, some asynchronous protocols can be modified to use committees. The challenge in asynchrony, with the lack of timeouts, is that no process can wait to hear from an entire committee nor can it wait for $n-f$ processes as usually done in such algorithms. Instead, some parameters are defined with respect to the system parameters such that safety and liveness can be provided with high probability.
Due to space limitations, we present here the parameters and guarantees as presented and proven in~\cite{cohen2020not} using Chernoff bounds. For simplicity, we only state the claims we are using in this paper.





\begin{namedtheorem}[Committee Sampling Properties from~\cite{cohen2020not}]
% All odd numbers are prime.

% \begin{theorem}

Let the set of processes sampled to the committee for $s$ and $\lambda$ be $C(s,\lambda)$, where $\lambda$ is set to $8\ln n$.
Let $d$ be a parameter of the system such that $\frac{1}{\lambda}<d < \frac{\epsilon}{3}-\frac{1}{3\lambda}$.
We set $W\triangleq \left \lceil{(\frac{2}{3}+3d)\lambda}\right \rceil$ and $B\triangleq \left \lfloor{(\frac{1}{3}-d)\lambda}\right \rfloor$.
With high probability the following hold:
\begin{description}
  \item[(S3)] At least
  $W$ processes in $C(s,\lambda)$ are correct.
    \item[(S4)] At most $B$ processes in $C(s,\lambda)$ are Byzantine.

    \item[(S5)] Consider $C(s,\lambda)$ for some string $s$ and two sets $P_1,P_2\subset C(s,\lambda)$ s.t $|P_1|=|P_2|=W$. Then, $|P_1\cap P_2|\geq B +1$.
\end{description}



% \end{theorem}
\end{namedtheorem}









% \subsection{Process replaceabilty}


% Process replaceabilty is a novel property, first presented in Algornad~\cite{Algorand} as \emph{player replaceabilty}.
% This property that was defined for a consensus protocol can be extended for all protocols using committees. As processes are sampled to participate in a committee randomly and independently (using VRF in this paper), one cannot predict which processes will act at any communication step of the protocol. As a result, Byzantine processes cannot cooperate between different steps of a protocol. Formally, process replaceabilty means that a protocol works correctly if a randomly and independently selected set of processes execute each communication step of the protocol.

% Achieving this property in our committee-based protocols allow us to treat the delayed-adaptive adversary as if it was static corruption. The adaptive adversary that does not know which processes participate in the protocol at each communication step has as much power as one who commits on corruption pattern at the beginning of the protocol. In order to achieve this property, each committee member sends at most one message before it ends its job. At that point, if the adversary decides to corrupt it, it doesn't affect the rest of the protocol.

==> sections/chernoff_proofs.tex <==
\section{Sampling proofs}
\label{chernoof_appendix}

\resampling*

\begin{proof}

Recall that $d$ is a parameter of the system such that $\max \{\frac{1}{\lambda},0.0362\}<d < \frac{\epsilon}{3}-\frac{1}{3\lambda}$.

In order to prove these properties we use two Chernoff bounds:

Suppose $X_1,...,X_n$ are independent random variables taking values in $\{0,1\}$. Let $X$ denote their sum and let $E[X]$ denote the sum's expected value.

\begin{equation}
\label{chernoff}
\forall 0 \leq \delta: \; Pr[X\geq (1+\delta)E[X]]\leq e^{-\frac{\delta ^2E[X]}{2+\delta}}
\end{equation}
\begin{equation}
\label{chernoff+}
\forall 0 \leq \delta\leq 1: \; Pr[X\leq (1-\delta)E[X]]\leq e^{-\frac{\delta ^2E[X]}{2}}
\end{equation}




\begin{lemma}[S1]
\label{comm_size_upper}
$|C(s,\lambda)|\leq (1+d)\lambda$ whp.
 \end{lemma}
\begin{proof}

Let $X$ be a random variable that represents the number of  processes that are sampled to $C(s,\lambda)$.
$X\sim Bin(n,\frac{const\cdot \ln n)}{n})$, thus $E[X]=const\cdot \ln n$.

Placing $\delta=d \geq 0$ in \ref{chernoff} we get:

\begin{equation*}
Pr[X\geq (1+d)const\cdot \ln n]\leq e^{-\frac{d^2const\cdot \ln n}{2+d}}.
\end{equation*}

Denote by $c_1$ the constant
$\frac{const\cdot d^2}{2+d}$. We get: 

\begin{equation*}
Pr[X\geq (1+d)const\cdot \ln n]\leq e^{-c_1\ln n}.
\end{equation*}

Thus, 
\begin{equation*}
Pr[X< (1+d)const\cdot \ln n]=Pr[X< (1+d)\lambda] > 1-\frac{1}{e^{c_1\ln n}}=1-\frac{1}{n^{c_1}}.
\end{equation*}

\end{proof}


\begin{lemma}[S2]
\label{comm_size_lower}
$|C(s,\lambda)|\geq (1-d)\lambda$ whp.
 \end{lemma}
\begin{proof}


Let $X$ be a random variable that represents the number of  processes that are sampled to $C(s,\lambda)$.
$X\sim Bin(n,\frac{const\cdot \ln n}{n})$, thus $E[X]=const\cdot \ln n$.

Placing $\delta=d $ it holds that $0\leq\delta\leq 1$ in \ref{chernoff+} and we get:

\begin{equation*}
Pr[X\geq (1-d)const\cdot \ln n]\leq e^{-\frac{d^2const\cdot \ln n}{2}}.
\end{equation*}

Denote by $c_2$ the constant
$\frac{const\cdot d^2}{2}$. We get: 

\begin{equation*}
Pr[X\geq (1-d)const\cdot \ln n]\leq e^{-c_2\ln n}.
\end{equation*}

Thus, 
\begin{equation*}
Pr[X<(1-d)const\cdot \ln n]=Pr[X< (1-d)\lambda] > 1-\frac{1}{e^{c_2\ln n}}=1-\frac{1}{n^{c_2}}.
\end{equation*}

\end{proof}





\begin{lemma}[S3]
At least $W$ processes in $C(s,\lambda)$ are correct whp.

\end{lemma}

\begin{proof}


Let $X$ be a random variable that represents the number of correct processes that are sampled to $C(s,\lambda)$.
$X\sim Bin((\frac{2}{3}+\epsilon)n,\frac{const\cdot \ln n}{n})$, thus $E[X]=(\frac{2}{3}+\epsilon)const\cdot \ln n$.
Let $d'=3d+\frac{1}{\lambda}$.
Notice that 
$1-\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon}\leq 1$ and also
$1-\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon}=1-\frac{\frac{2}{3}+3d+\frac{1}{\lambda}}{\frac{2}{3}+\epsilon}=\frac{\frac{2}{3}+\epsilon-\frac{2}{3}-3d-\frac{1}{\lambda}}{\frac{2}{3}+\epsilon} \geq
\frac{\frac{3}{\lambda}+\frac{1}{\lambda}-3d-\frac{1}{\lambda}}{\frac{2}{3}+\epsilon}
\geq 0$.
Hence, we can put $\delta=1-\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon}$ in (\ref{chernoff+}) and get:



\begin{equation*}
Pr[X\leq (1-(1-\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon}))(\frac{2}{3}+\epsilon)const\cdot \ln n]\leq e^{-\frac{(1-\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon}) ^2(\frac{2}{3}+\epsilon)const\cdot \ln n}{2}},
\end{equation*}


\begin{equation*}
Pr[X\leq (\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon})(\frac{2}{3}+\epsilon)const\cdot \ln n]\leq e^{-\frac{(1-\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon}) ^2(\frac{2}{3}+\epsilon)const\cdot \ln n}{2}},
\end{equation*}


\begin{equation*}
Pr[X\leq (\frac{2}{3}+d')const\cdot \ln n]\leq e^{-\frac{(1-\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon}) ^2(\frac{2}{3}+\epsilon)const\cdot \ln n}{2}}.
\end{equation*}

Denote by $c_3$ the constant $\frac{const\cdot (1-\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon}) ^2(\frac{2}{3}+\epsilon)}{2}$. We get: 

\begin{equation*}
Pr[X\leq (\frac{2}{3}+d')const\cdot \ln n]\leq e^{-c_3\ln n}.
\end{equation*}

Thus, 
\begin{equation*}
Pr[X> (\frac{2}{3}+d')const\cdot \ln n]=Pr[X> (\frac{2}{3}+d')\lambda] > 1-\frac{1}{e^{c_3\ln n}}=1-\frac{1}{n^{c_3}}.
\end{equation*}

To this point we've proved that at least
  $(\frac{2}{3}+d')\lambda$ processes in $C(s,\lambda)$ are correct whp. It follows that at least
  $(\frac{2}{3}+3d+\frac{1}{\lambda})\lambda=(\frac{2}{3}+3d)\lambda+1$ processes in $C(s,\lambda)$ are correct whp.
  
  
  As $\left \lceil{(\frac{2}{3}+3d)\lambda}\right \rceil \leq (\frac{2}{3}+3d)\lambda+1$ we conclude that at least
  $W=\left \lceil{(\frac{2}{3}+3d)\lambda}\right \rceil$ processes in $C(s,\lambda)$ are correct whp.


\end{proof}


\begin{lemma}[S4]
 At most $B$ processes in $C(s,\lambda)$ are Byzantine whp.
\end{lemma}
\begin{proof}

Let $X$ be a random variable that represents the number of Byzantine processes that are sampled to $C(s,\lambda)$.
$X\sim Bin((\frac{1}{3}-\epsilon)n,\frac{const\cdot \ln n}{n})$, thus $E[X]=(\frac{1}{3}-\epsilon)const\cdot \ln n$.

Placing $\delta=\frac{\epsilon-d}{\frac{1}{3}-\epsilon}\geq 0$ in (\ref{chernoff}) we get:

\begin{equation*}
Pr[X\geq (1+\frac{\epsilon-d}{\frac{1}{3}-\epsilon})(\frac{1}{3}-\epsilon)const\cdot \ln n]\leq e^{-\frac{(\frac{\epsilon-d}{\frac{1}{3}-\epsilon})^2(\frac{1}{3}-\epsilon)const\cdot \ln n}{2+(\frac{\epsilon-d}{\frac{1}{3}-\epsilon})}},
\end{equation*}
\begin{equation*}
Pr[X\geq (\frac{\frac{1}{3}-d}{\frac{1}{3}-\epsilon})(\frac{1}{3}-\epsilon)const\cdot \ln n]\leq e^{-\frac{\frac{(\epsilon-d)^2}{\frac{1}{3}-\epsilon}const\cdot \ln n}{2+(\frac{\epsilon-d}{\frac{1}{3}-\epsilon})}},
\end{equation*}
\begin{equation*}
Pr[X\geq (\frac{1}{3}-d)const\cdot \ln n]\leq e^{-\frac{\frac{(\epsilon-d)^2}{\frac{1}{3}-\epsilon}const\cdot \ln n}{2+(\frac{\epsilon-d}{\frac{1}{3}-\epsilon})}}.
\end{equation*}

Denote by $c_4$ the constant
${\frac{const\cdot \frac{(\epsilon-d)^2}{\frac{1}{3}-\epsilon}}{2+(\frac{\epsilon-d}{\frac{1}{3}-\epsilon})}}$. We get: 

\begin{equation*}
Pr[X\geq (\frac{1}{3}-d)const\cdot \ln n]\leq e^{-c_4\ln n}.
\end{equation*}

Thus, 
\begin{equation*}
Pr[X< (\frac{1}{3}-d)const\cdot \ln n]=Pr[X< (\frac{1}{3}-d)\lambda] > 1-\frac{1}{e^{c_4\ln n}}=1-\frac{1}{n^{c_4}}.
\end{equation*}


Since X must be an integer, it follows that $X\leq B=\left \lfloor{(\frac{1}{3}-d)\lambda}\right \rfloor$ whp.


\end{proof}






% \begin{lemma}[S9]
%  At most $(\frac{1}{3}-d)\lambda-2$ processes in $C$ are Byzantine w.h.p.
% \end{lemma}
% \begin{proof}

% Let $X$ be a random variable that represents the number of Byzantine processes that are sampled to $C$.
% $X\sim Bin((\frac{1}{3}-\epsilon)n,\frac{\ln n}{n})$, thus $E[X]=(\frac{1}{3}-\epsilon)\ln n$.



% Let $d'=d+\frac{2}{\lambda}$.

% Placing $\delta=\frac{\epsilon-d'}{\frac{1}{3}-\epsilon}\geq 0$ in (\ref{chernoff}) we get:

% % Notice that 
% % $1-\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon}\leq 1$ and since $\epsilon> \frac{3}{\lambda}$ also
% % $1-\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon}\geq 0$.
% % Hence, we can put $\delta=1-\frac{\frac{2}{3}+d'}{\frac{2}{3}+\epsilon}$ in (\ref{chernoff+}) and get:


% \begin{equation*}
% Pr[X\geq (1+\frac{\epsilon-d}{\frac{1}{3}-\epsilon})(\frac{1}{3}-\epsilon)\ln n]\leq e^{-\frac{(\frac{\epsilon-d}{\frac{1}{3}-\epsilon})^2(\frac{1}{3}-\epsilon)\ln n}{2+(\frac{\epsilon-d}{\frac{1}{3}-\epsilon})}},
% \end{equation*}
% \begin{equation*}
% Pr[X\geq (\frac{\frac{1}{3}-d}{\frac{1}{3}-\epsilon})(\frac{1}{3}-\epsilon)\ln n]\leq e^{-\frac{\frac{(\epsilon-d)^2}{\frac{1}{3}-\epsilon}\ln n}{2+(\frac{\epsilon-d}{\frac{1}{3}-\epsilon})}},
% \end{equation*}
% \begin{equation*}
% Pr[X\geq (\frac{1}{3}-d)\ln n]\leq e^{-\frac{\frac{(\epsilon-d)^2}{\frac{1}{3}-\epsilon}\ln n}{2+(\frac{\epsilon-d}{\frac{1}{3}-\epsilon})}}.
% \end{equation*}

% Denote by $c_4$ the constant
% ${\frac{\frac{(\epsilon-d)^2}{\frac{1}{3}-\epsilon}}{2+(\frac{\epsilon-d}{\frac{1}{3}-\epsilon})}}$. We get: 

% \begin{equation*}
% Pr[X\geq (\frac{1}{3}-d)\ln n]\leq e^{-c_4\ln n}.
% \end{equation*}

% Thus, 
% \begin{equation*}
% Pr[X< (\frac{1}{3}-d)\ln n]=Pr[X< (\frac{1}{3}-d)\lambda] > 1-\frac{1}{e^{c_4\ln n}}=1-\frac{1}{n^{c_4}}.
% \end{equation*}


% \end{proof}


\end{proof}


\WW*

\begin{proof}
The set $P_2$ contains at most $|C(s,\lambda)\setminus P_1|$ processes that aren't in $P_1$. By S1, and since $P_1\subset C(s,\lambda)$:
\begin{equation*}
|C(s,\lambda)\setminus P_1|\leq
(1+d)\lambda-W =
(1+d)\lambda-\left \lceil{(\frac{2}{3}+3d)\lambda}\right \rceil \leq (1+d)\lambda-(\frac{2}{3}+3d)\lambda = (\frac{1}{3}-2d)\lambda.
\end{equation*}

The remaining processes in $P_2$ are also in $P_1$, so

\begin{equation*}
|P_1\cap P_2|\geq 
W-(\frac{1}{3}-2d)\lambda=
\left \lceil{(\frac{2}{3}+3d)\lambda}\right \rceil -(\frac{1}{3}-2d)\lambda
\geq 
(\frac{2}{3}+3d)\lambda -(\frac{1}{3}-2d)\lambda= (\frac{1}{3}+5d)\lambda.
\end{equation*}
Finally, 

\begin{equation*}
|P_1\cap P_2|-B =
|P_1\cap P_2|-\left \lfloor{(\frac{1}{3}-d)\lambda}\right \rfloor\geq (\frac{1}{3}+5d)\lambda-(\frac{1}{3}-d)\lambda=6d\lambda>\frac{6\lambda}{\lambda} \geq 1,
\end{equation*}

as requested.
\end{proof}

\WB*

\begin{proof}
    
The set $P_2$ contains at most $|C(s,\lambda)\setminus P_1|$ processes that aren't in $P_1$. By S1, and since $P_1\subset C(s,\lambda)$:
\begin{equation*}
|C(s,\lambda)\setminus P_1|\leq
(1+d)\lambda-(B+1) =
(1+d)\lambda-(\left \lfloor{(\frac{1}{3}-d)\lambda}\right \rfloor+1)
\leq
(1+d)\lambda-((\frac{1}{3}-d)\lambda-1)-1
=(\frac{2}{3}+2d)\lambda.
\end{equation*}

Therefore,

\begin{equation*}
|P_2|-|C(s,\lambda)\setminus P_1|\geq 
W-(\frac{2}{3}+2d)\lambda=
\left \lceil{(\frac{2}{3}+3d)\lambda}\right \rceil-(\frac{2}{3}+2d)\lambda
\geq
{(\frac{2}{3}+3d)\lambda}-(\frac{2}{3}+2d)\lambda
=d\lambda >\frac{\lambda}{\lambda}=1 ,
\end{equation*}




and so $|P_1\cap P_2|\geq 1$, as requested.
\end{proof}



==> sections/consensus.tex <==
\section{Asynchronous sub-quadratic Byzantine Agreement}
\label{sec:consensus}

We adapt the Byzantine Agreement algorithm of Mostefaoui et al.~\cite{mostefaoui2015signature} to work with committees. Our protocol leverages 
an \emph{approver} abstraction, which we implement in Section \ref{sec:approver} and then integrate it into a Byzantine Agreement protocol in Section \ref{sec:consensus_protocol}. 

% As we will explain later, the \emph{ratifier} allow process replaceability while using committees.



\input{sections/ratifier.tex}

\input{sections/consensus_whp.tex}


% \label{sec:consensus_protocol}

We present the pseudo-code for our algorithm in Algorithm \ref{alg:consensus_protocol}.
Our protocol executes in rounds. Each round consists of two approver invocations and one call to the WHP coin.
Again, we discuss the algorithm assuming S1-S6 hold. We will argue that the algorithm decides in a constant number of rounds whp, and so these properties hold for all the committees it uses.
The local variable $est_i$ holds $p_i$'s current estimate of the decision value. The variable $decision_i$ holds $p_i$'s irrevocable decision. It is initialized to $\bot$ and set to a value in $\{0,1\}$ at most once.
Every process $p_i$ begins by setting $est_i$ to hold its initial value.
At the beginning of each round processes execute the approver with their $est$ values. If they return a singleton $\{v\}$, they choose to invoke the next approver with $v$ as their proposal and otherwise they invoke the next approver with $\bot$.
By the approver's graded agreement property, different processes do not return different singletons. Thus, at most two different values ($\bot$ and one in $\{0,1\}$) are given as an input by correct processes to the next approver, satisfying Assumption \ref{two_values}.



At this point, after all correct processes have chosen their proposals, they all invoke the WHP coin in line \ref{l.con.coin} in order to select a fall-back value. Notice that executing the WHP coin protocol after proposals have been set prevents the adversary from biasing proposals based on the coin flip. Then, in in line \ref{l.con.app2}, all processes invoke the approver with their proposals. If a process does not receive $\bot$ in its return set, it can safely decide the value it received. It does so by updating its $decision$ variable in line \ref{l.con.decide}. If it receives some value other than $\bot$ it adopts it to be its estimated value (line \ref{l.con.update_est3}), whereas if it receives only $\bot$, it adopts the coin flip (line \ref{l.con.update_est2}).
If all processes receive $\bot$ in line \ref{l.con.app1} then the probability that they all adopt the same value is at least $2\rho$, where $\rho$ is the coin's success rate. If some processes receive $v$, then the probability that all the processes that adopt the coin flip adopt $v$ is at least $\rho$.
With high probability, after a constant number of rounds, all correct processes have the same estimated value. By validity of the approver, once they all have common estimate, they decide upon it within 1 round.

\input{sections/consensus_protocol.tex}



We now prove our main theorem:

\begin{theorem}
\label{main_theo}
Algorithm~\ref{alg:consensus_protocol} when using an approver (Definition \ref{def:approver}) and a WHP coin (Definition \ref{def:whp_coin})
solves Byzantine Agreement whp (Definition \ref{def:consensus_whp}).
\end{theorem}


\input{sections/consensus_whp_proofs.tex}




% \paragraph{Complexity}
{\bf Complexity.} 
In each round of the protocol, all correct processes invoke two approver calls and one WHP coin instance. Due to the constant success rate of the WHP coin, the expected number of rounds before all correct processes decide is constant. Thus, due to the word complexity of the WHP coin and approver, the expected word complexity is $O(n\log^2 n)=\widetilde{O}(n)$ and the time complexity is $O(1)$ in expectation.




==> sections/consensus_proofs.tex <==


% \begin{lemma}{(Validity)}
% \label{validity}
% If at the beginning of phase $r$ all correct processes have the same estimate value $v$, then any correct process that has not decided before decides $v$ by the end of phase $r$.
% \end{lemma}
% \begin{proof}
% If all correct processes starts phase $r$ with the same estimate value $v$, they all execute ratify($v$). Hence, by ratifier's validity and termination, they all return the non-empty set $\{v\}$ and update their $propose$ value to $v$. Then, they all execute ratify($v$) for the second time and due to the same reason they all return $\{v\}$. By the protocol, any correct process that has not decided before decides $v$ at line 13.
% \end{proof}

% \begin{lemma}{(Agreement)}
% \label{agreement}
% No two correct processes decide different values.
% \end{lemma}
% \begin{proof}
% Let $r$ be the first phase in which a process $p_1$ decides on some value $v$. Thus, $p_1$'s invocation to ratifier in line $9$ of phase $r$ returns $\{v\}$ for $v\neq \bot$. If another correct process $p_2$ also decides in phase $r$ then its ratifier call in line $9$ of phase $r$ returns $\{w\neq \bot\}$. By ratifier's graded agreement $v=w$.
% Consider a correct process $p_3$ that does not decide in phase $r$. By the definition of $r$, $p_3$ hasn't decided in any phase $r'<r$. By ratifier's graded agreement, $p_3$ returns $\{v,\bot\}$ in line $9$ of phase $r$. Thus, $p_3$ updates its $est_p$ value to $v$ in line 18.
% It follows that all correct processes have $v$ as their estimate value in the beginning of phase $r+1$. By Lemma \ref{validity} every correct process that has not decided in phase $r$ decides $v$ in phase $r+1$.
% \end{proof}


% \begin{lemma}
% \label{liveness}
% No correct process remains blocked forever during a phase $r$.
% \end{lemma}
% \begin{proof}
% \shir{still not sure about this proof}

% We show by induction on the phase number $r$ that if all correct process start executing phase $r$, then they all proceeds to phase $r+1$.

% The basis is $r=0$
% The only waits in the protocol is while executing the ratifier and the shared coin primitives (in lines 4,8,9). If all correct process invoke the shared coin and ratifier primitives then their termination property hold and they all return from the call. Thus, since all correct processes start executing the same code in phase $0$, they all return in line 4. Then, they all return in line 8 and in line 9, and proceed to phase $1$.

% Suppose the claim is true for phase $r-1\geq 0$. Thus, if all correct process start executing phase $r-1$ they all proceed to phase $r$. The same reasoning as in the basis applies for phase $r$ and all correct processes proceed to phase $r+1$.

% Therefore, no correct process remains blocked forever during a phase $r$.
% \end{proof}


% \begin{lemma}
% \label{termination}
% Every correct process decides with probability 1.
% \end{lemma}
% \begin{proof}
% Consider phase $r$ of the protocol. By Lemma \ref{liveness} all correct process
% reaches phase $r$ and executes it fully. 
% We examine all possible scenarios in phase $r$:
% \begin{enumerate}
%     \item All correct processes return $\{v\}$ in line 4:
    
%     By ratifier's graded agreement they return $\{v\}$ with the same value $v$. Hence, all correct processes update their $propose$ value to $v$. Then, they all execute ratify($v$) in line 9 and by graded agreement they all return $\{v\}$. By the protocol, they all decide $v$ with probability 1 (if haven't decided yet).
    
%     \item
%     All correct processes return $\{v,\bot\}$ in line 4:
    
%     All correct processes update their $propose$ value to $\bot$. Then,
%     they all execute ratify($\bot$) in line 9 and by graded agreement they  return $\{\bot\}$. By the protocol, all correct processes update their estimate value to the coin toss of the shared coin. With probability $\psi \geq 2\rho$, where $\rho$ is the defiance of the shared coin, all correct processes toss the same $v\in \{0,1\}$. By Lemma \ref{validity}, in phase $r+1$ they all decide $v$ with probability $\psi$ (if haven't decided yet).
%     \shir{we need to mention somewhere that at every phase, the first values that correct processes ratify is indeed 0/1 because we solve binary consensus. otherwise, the coin toss has no meaning. I'm not sure where to mention it}
    
%     % If a correct process decided $v$ before phase $r$, then by Lemma \ref{agreement} no correct process has decided $w\neq v$.
    

    
    
%     \item At least one correct process, but not all correct processes, returns $\{v\}$ in line 4:
    
    
%     We'll examine two possible complementary sub-cases:
    
%     \begin{itemize}
%         \item If a correct process returns $\{v\neq \bot\}$ in line 9:
%         By ratifier's graded agreement no correct process returns $\{\bot\}$ in line 9. Thus, all correct processes update their estimate value to $v$ (in line 11/18). By Lemma \ref{validity}, in phase $r+1$ they all decide $v$ with probability 1 (if haven't decided yet).
        
        
%         \item If no correct process returns $\{v\neq \bot\}$ in line 9:
%         All correct processes either update their estimate value to the coin toss of the shared coin (line 16) or to the same value $v\neq \bot$ (line 18).
%         As the set $props$ contains at most two values, all correct processes that update their value in line 18 update the same value. Since the value $v$ is determined before tossing the coin, the adversary cannot bias $v$ after viewing the coin toss and with probability $\psi \geq \rho$, where $\rho$ is the defiance of the shared coin, all correct processes that adopt the coin's value will toss $v$. By Lemma \ref{validity}, in phase $r+1$ all correct processes decide $v$ with probability $\psi$ (if haven't decided yet).
    
    
%     \end{itemize}

    
% \end{enumerate}

% In all cases, with probability greater than $\rho$ all correct processes decide by phase $r+1$. The probability of not terminating is $\lim_{r\to\infty} (1-\rho)^r$, which equals 0 using our shared coin.	

% \end{proof}


\begin{theorem}
 Algorithm~\ref{alg:consensus_protocol}
solves randomized byzantine binary consensus.
\end{theorem}


\begin{proof}

If all correct processes start with value $v$ then, by Lemma \ref{validity}, they all decide $v$ and validity holds. Agreement follows from Lemma \ref{agreement} and termination follows from Lemma \ref{termination}.

% \begin{description}
% \item[] We show that the protocol satisfies the validity, agreement, and termination properties:
%   \item[Validity]
%   If all correct processes start with value $v$ then, by Lemma \ref{validity}, they all decide $v$.
%   \item[Agreement]
%   Follows from Lemma \ref{agreement}.
%   \item[Termination]
%   Follows from Lemma \ref{termination}.
% \end{description}
\end{proof}

==> sections/consensus_protocol.tex <==




\begin{algorithm}
\caption{Protocol Byzantine Agreement($v_i$): code for process $p_i$}

\begin{multicols}{2}

\begin{algorithmic}[1]


\State  $est_i \gets v_i$
\State $decision_i\gets \bot$
\Statex


\For{$r=0,1,...$}

\State  $vals \gets$ approve($est_i$) \label{l.con.app1}
\If{$vals=\{v\}$ for some $v$}
\State $propose_i\gets v$ \label{l.con.update_propose}
% \Else    $propose_i\gets \bot$
\EndIf
\State \textbf{otherwise} $propose_i\gets \bot$
\Statex


\State $c \gets $ whp\textunderscore coin($r$) \label{l.con.coin}
\State  $props \gets$ approve($propose_i$) \label{l.con.app2}
\If{$props=\{v\}$ for some $v\neq \bot$}
\State $est_i\gets v$ \label{l.con.update_est1}

\If{$decision_i=\bot$}
\State $decision_i\gets v$ \label{l.con.decide}
\EndIf

\Else \If{$props=\{ \bot\}$}
\State $est_i\gets c$ \label{l.con.update_est2}

\Else \Comment{$props=\{v,\bot \}$}
\State $est_i \gets v$ \label{l.con.update_est3}

\EndIf
\EndIf
\EndFor

\end{algorithmic}
\end{multicols}
\label{alg:consensus_protocol}
\end{algorithm}




==> sections/consensus_whp.tex <==
\subsection{Byzantine Agreement WHP}
\label{sec:consensus_protocol}
Our next step is solving Byzantine Agreement whp, formally defined as follows:


\begin{definition}[Byzantine Agreement WHP]
\label{def:consensus_whp}
In Byzantine Agreement WHP, each correct process $p_i\in\Pi$ proposes a binary input value $v_i$ and decide on an output value $decision_i$ s.t. with high probability the following properties hold:


\begin{itemize}
    \item Validity. If all correct processes propose the same value $v$, then any correct process
that decides, decides $v$.
    \item Agreement. No two correct processes decide differently.
    \item Termination. Every correct process eventually decides.
\end{itemize}

\end{definition}




==> sections/consensus_whp_proofs.tex <==


We first show that Algorithm \ref{alg:consensus_protocol} satisfies the approver and WHP coin primitives' assumptions whp. Proving this allows us to use their properties while proving Theorem \ref{main_theo}.


\begin{lemma}
\label{correct_use_of_primitives}
For every round $r$ of Algorithm \ref{alg:consensus_protocol} the following hold:
\begin{enumerate}
\item All correct processes invoke approve with at most 2 different values.
\item The invocation of whp\textunderscore coin$(r)$ by a correct process $p$ is causally independent of its progress at other processes.
\end{enumerate}


\end{lemma}
\begin{proof}
\begin{enumerate}
\item It is easy to see, by induction on the number of rounds, that since the processes' inputs are binary and we use a binary coin, the $est$ of all processes is in $\{0,1\}$ at the beginning of each round. Hence, the approver in line \ref{l.con.app1} is invoked with at most two different values. Due to its graded agreement property, all processes that update their propose to $v\neq \bot$ in line \ref{l.con.update_propose} update it to the same value whp. Thus, whp, in line \ref{l.con.app2} approver is invoked with either $v$ or $\bot$.


\item Correct processes call $whp$\textunderscore $coin(r)$ without waiting for indication that other processes have done so.
\end{enumerate}
\end{proof}


Next, we show that for any given round of the algorithm, (1) whp all processes complete this round, and (2) with a constant probability, they all have the same estimate value by its end.

\begin{lemma}
\label{complete_same_est}
If all correct processes begin round $r$ of Algorithm \ref{alg:consensus_protocol} then whp:
\begin{enumerate}
    \item All correct processes complete round $r$, i.e. they're not blocked during round $r$. \label{complete_same_est_1}
    \item With probability greater than $\rho$, where $\rho$ is the success rate of the WHP coin, all correct processes have the same $est$ value at the end of round $r$. \label{complete_same_est_2}
\end{enumerate}

\end{lemma}
\begin{proof}
First, if all correct processes begin round $r$ then they all invoke the approver in line \ref{l.con.app1}. Their invocation returns whp so they all invoke the coin in line \ref{l.con.coin}, and so it returns and all invoke approve in line \ref{l.con.app2}, and so it also returns, proving~(\ref{complete_same_est_1}). To show~(\ref{complete_same_est_2}), consider the possible scenarios with respect to the approver's return value:
\begin{itemize}
    \item All correct processes return singletons in line \ref{l.con.app1}:
    
    By the approver's graded agreement, whp they return $\{v\}$ with the same value $v$. Hence, all correct processes update their $propose$ to $v$. Then, they all execute approve($v$) in line \ref{l.con.app2}, and by validity, they all return $\{v\}$ whp. In this case they all update $est\gets v$.
    
    \item
    All correct processes return $\{0,1\}$ in line \ref{l.con.app1}:
    
    All correct processes update their $propose$ value to $\bot$. Then,
    they all execute approve($\bot$) in line \ref{l.con.app2}, and by validity, they  return $\{\bot\}$ whp. In this case, all correct processes then update their estimate value to the coin flip (line \ref{l.con.update_est2}). With probability at least $2\rho$ all correct processes toss the same $v\in \{0,1\}$.
    
    
    \item Some, but not all correct processes return singletons in line \ref{l.con.app1}:
    
    By graded agreement, all singletons hold the same value $v$. Thus, all correct processes propose $v$ or $\bot$ and by validity return $\{v\}, \{v,\bot\}$, or $\{\bot\}$ in line \ref{l.con.app2}.
    We examine two possible complementary sub-cases:
    
    \begin{itemize}
        \item If some correct process returns $\{v\}$ in line \ref{l.con.app2}:
        By approver's graded agreement, no correct process returns $\{\bot\}$ in line \ref{l.con.app2}, whp. Thus, whp, all correct processes update their estimate value to $v$ (in line \ref{l.con.update_est1} or \ref{l.con.update_est3}).
        
        \item If no correct process return $\{v\}$ in line \ref{l.con.app2}:
        All correct processes returns $\{v,\bot\}$ or $\{\bot\}$ in line \ref{l.con.app2}.
        All correct processes either update their estimate value to the coin flip of the WHP coin (line \ref{l.con.update_est2}) or to $v$ (line \ref{l.con.update_est3}). Since the value $v$ is determined before tossing the coin, the adversary cannot bias $v$ after viewing the coin flip and with probability at least $\rho$ all correct processes that adopt the coin's value toss $v$.
        
    \end{itemize}
\end{itemize}


In all cases, with probability greater than $\rho$ all correct processes have the same $est$ value at the end of $r$, whp.
\end{proof}


The following lemmas indicate that the Byzantine Agreement whp properties are satisfied, which completes the proof of Theorem \ref{main_theo}.


\begin{lemma}{(Validity)}
\label{validity_whp}
If at the beginning of round $r$ of Algorithm \ref{alg:consensus_protocol} all correct processes have the same estimate value $v$, then whp any correct process that has not decided before decides $v$ in round $r$.
\end{lemma}
\begin{proof}
If all correct processes start round $r$ then by Lemma \ref{complete_same_est} they all complete round $r$. Since they all being with the same estimate value $v$, they all execute approve($v$) in line \ref{l.con.app1}. Hence, by approver's validity and termination, whp they all return the non-empty set $\{v\}$ and update their $propose$ values to $v$. Then, they all execute approve($v$) for the second time in line \ref{l.con.app2}, and due to the same reason, they all return $\{v\}$ whp. Any correct process that has not decided before decides $v$ in line \ref{l.con.decide}.
\end{proof}

\begin{lemma}{(Termination)}
\label{termination_whp}
Every correct process decides whp.

\end{lemma}
\begin{proof}

By Lemma \ref{complete_same_est}, for every round $r$ of Algorithm \ref{alg:consensus_protocol}, with probability greater than $\rho$, where $\rho$ is the success rate of the WHP coin, all correct processes have the same $est$ value at the end of $r$ whp.
Hence, by Lemma \ref{validity_whp}, with probability greater than $\rho$, all correct processes decide by round $r+1$ whp. 
It follows that the expected number of rounds until all processes decide is bounded by $\frac{1}{\rho}$, which is constant.
Thus, by Chebyshev's inequality, whp all correct processes decide within a constant number of rounds.
\end{proof}


 


\begin{lemma}{(Agreement)}
\label{agreement_whp}
No two correct processes decide different values whp.
\end{lemma}
\begin{proof}
Let $r$ be the first round in which some process $p_i$ decides on some value $v\in \{0,1\}$. Thus, $p_i$'s invocation to approver in line \ref{l.con.app2} of round $r$ returns $\{v\}$. If another correct process $p_j$ decides $w$ in round $r$ then its approver call in line \ref{l.con.app2} of round $r$ returns $\{w\}$. By approver's graded agreement, $v=w$ whp.
Consider a correct process $p_k$ that does not decide in round $r$. By the definition of $r$, $p_k$ hasn't decided in any round $r'<r$. By approver's graded agreement, whp, $p_k$ returns $\{v,\bot\}$ in line \ref{l.con.app2} of round $r$, and $p_k$ updates its $est_{k}$ value to $v$ in line \ref{l.con.update_est3}.
It follows that whp all correct processes have $v$ as their estimate value at the beginning of round $r+1$. By Lemma \ref{validity_whp}, every correct process that has not decided in round $r$ decides $v$ in round $r+1$ whp.
\end{proof}


==> sections/multivalue_proofs.tex <==

\subsection{Correctness Proof}
\label{subsec:proof}


\begin{lemma}{(Validity)}
If all processes are correct and they all propose the same value $v$, then they all decide $v$ WHP.
\end{lemma}
\begin{proof}

If all processes are correct and propose the same value $v$, then all members of the \textsc{init} committee broadcast $v$. By S3, WHP, there are at least $W$ correct processes in the \textsc{init} committee. Hence, every process in the \textsc{converge} committee receives $W$ \textsc{init} messages with the value $v$ and by assumption $v$ is its initial value. Thus, WHP all correct processes in the \textsc{converge} committee execute lines~\ref{l:batch_qc} -- \ref{l:send_qc} and send a \textsc{converge} message with a quorum certificate on $v$.

By S3, WHP, there are at least $W$ correct processes in the \textsc{converge} committee.
Hence, all correct processes receive $W$ \textsc{converge} messages with a $\emph{is\_content}=true$ and a quorum certificate on $v$, for each of them they increase the counter at line~\ref{l:inc_counter}.
Following that, and since $W>B$, all correct processes set alert to \emph{false} at line~\ref{l:check_count} and start the binary BA with the same input \emph{false}.
By the strong unanimity validity condition of the binary BA, they all decide on \emph{false} at line~\ref{l:binary_dec}.
Since they all previously received a \textsc{converge} messages with a quorum certificate on $v$, they all decide on $v$ at line~\ref{l:dec_by_qc}.


% values that are not $v$, and send a <converge,false> message to all processes accordingly at line 9. In addition, none of them changes the content flag, and thus all correct processes have content set to true, as it is initialized.

% As a result, and since there are at most $B$ Byzantine in the converge committee, all correct processes then receive at most B <converge,true> messages. Thus, the counter can be updated at most $B$ times at line 12. As a result, all correct processes update alert to false at line 14 and invoke the binary BA at line 15 with the same initial value. By Theorem~\ref{main_theo}, they all decide alert false. Then, they all perform line 21, and as their content flag is set to true, they all decide their inital value $v$.
\end{proof}



\begin{lemma}
\label{lemma:evn_qc}
If the binary decision is \emph{false} at line~\ref{l:binary_dec}, then all correct processes receive a message $\lr{\textsc{converge},\emph{true},QC_{v}}_j$ from validly sampled $p_j$ WHP.
\end{lemma}
\begin{proof}
Notice that there exists at least one correct process $p_i$ that initiates the binary agreement with $alert=false$, as otherwise by the strong unanimity validity condition of the binary BA the binary decision must have been true. It follows from the code (line~\ref{l:inc_counter}, \ref{l:check_count}) that $p_i$ received at least $B+1$ \textsc{converge} messages with \emph{is\_content=true}. By property S4, WHP, there are at most $B$ Byzantine processes in the \textsc{converge} committee. Hence, $p_i$ received the \textsc{converge} message with a QC from at least one correct process $p_j$. By the code, $p_j$ must have sent that message to all correct processes at line~\ref{l:send_qc}. Therefore, every correct process eventually receives that message.

% and can decide safely at line~\ref{l:dec_by_qc}.
\end{proof} 


\begin{lemma}{(Termination)}
Every correct process decides WHP.

\end{lemma}
\begin{proof}
By S3, WHP, $W$ correct processes are elected to the \textsc{init} committee, broadcasting an \textsc{init} message. Thus, every correct process who is sampled to the \textsc{converge} committee eventually receives W \textsc{init} messages WHP and enters the if condition at line~\ref{l:terminate_init}. By S3 again, WHP, at least $W$ correct processes are elected to the \textsc{converge} committee. Thus, every correct process receives WHP $W$ \textsc{converge} messages, and execute line~\ref{l:terminate_converge}. By the termination of the binary BA, all correct processes terminate the binary BA WHP.
If the binary decision is \emph{true}, then they all decide at line~\ref{l:dec_def}. Otherwise, by Lemma~\ref{lemma:evn_qc} they all decide at line~\ref{l:dec_by_qc} after receiving a valid $\lr{\textsc{converge},\emph{true},QC_{v}}_j$ message WHP.
\end{proof}




\begin{lemma}{(Agreement)}
No two correct processes decide different values WHP.
\end{lemma}
\begin{proof}
According to the binary BA agreement, all correct processes decide the same value WHP at line~\ref{l:binary_dec}.
We consider the two possible binary BA outputs.
If the binary decision is \emph{true}, then all correct processes decide the domain's default value, and hence the same value. 
Otherwise, the binary decision is \emph{false} and the decision is made according to the value signed in a QC received in a converge message. By Lemma~\ref{lemma:evn_qc}, WHP all correct processes receive a converge message with \emph{is\_content} flag set to \emph{true}. It is left to show that all of these messages carry a quorum certificate for the same value $v$.

A valid QC on value $v$ is created by aggregated signatures of $W$ different processes who sent an \textsc{init} message on the value $v$. By property S5, every two subsets of the \textsc{init} committee of size $W$ intersect by at least one correct process. Since a correct process only signs one \textsc{init} message it follows that only one valid QC can be sent at line~\ref{l:send_qc}.


\end{proof}



% \subsection{Complexity}
\textbf{Complexity.}
In Algorithm~\ref{alg:to_multi} all correct processes that are sampled to the two committees (lines~\ref{l:send_init},\ref{l:terminate_init}) send messages to all other processes.
The committee size is $O(\lambda)=O(\log n)$ WHP.
Each of these messages contains a value from the finite domain and a VRF proof of the sender’s election to the committee. In addition, a message possibly contains a quorum certificate of $O(\lambda)$ committee members' messages.
Therefore, each message's size is at most $O(\lambda)$ words, and  the total word complexity of a multivalued weak BA WHP is $O(n\lambda^2)=O(n\log^2 n)=\widetilde{O}(n)$ in expectation.



We conclude:

\begin{theorem}
Algorithm~\ref{alg:to_multi} implements multivalued weak Byzantine Agreement WHP with a word complexity of $\widetilde{O}(n)$.
\end{theorem} 

% \label{subsec:complexity}


==> sections/related_work.tex <==
\section{Related Work}
\label{sec:related_work}


% \paragraph{Lower bounds.}
{\bf Lower bounds.} 
Our assumptions conform with a number of known bounds. Deterministic consensus is impossible in an asynchronous system if even one process may crash (by FLP~\cite{fischer1985impossibility}) and requires $\Omega(n^2)$ communication even in synchronous systems~\cite{DolevBound}. As for randomized Byzantine Agreement, Abraham et al.
\cite{abraham2019communication} state that disallowing
after-the-fact removal is necessary even in synchronous settings for achieving sub-quadratic communication.

% \paragraph{Asynchronous BA and shared coin algorithms.}
{\bf Asynchronous BA and shared coin algorithms.} 
The algorithms we present in this paper belong to the family of asynchronous BA algorithms, which sacrifice determinism in order to circumvent FLP. We compare our solutions to existing ones in Table~\ref{tab:survey}.
 
Ben-Or~\cite{ben1983another} suggested a protocol with resilience $n>5f$. This protocol uses a local coin (namely, a local source of randomness) and its expected time complexity is exponential (or constant if $f=O(\sqrt n)$). Bracha~\cite{bracha1987asynchronous} improved the resilience to $n>3f$ with the same complexity. The complexity can be greatly reduced by replacing the local coin with a shared one with a guaranteed success rate.

Later works presented the shared coin abstraction and used it to solve BA with $O(n^2)$ communication. Rabin~\cite{rabin1983randomized} was the first to do so, suggesting a protocol with resilience $n>10f$ and a constant expected number of rounds. Cachin et al.~\cite{cachin2005random} were the first to use a shared coin to solve BA with $O(n^2)$ communication and optimal resilience.
Mostefaoui et al.~\cite{mostefaoui2015signature} then presented a signature-free BA algorithm with optimal resilience and $O(n^2)$ messages that uses a shared coin abstraction as a black box; the shared coin algorithm we provide in Section 4 can be used to instantiate this protocol. All of the aforementioned algorithms solve binary BA, where the processes’ initial values are 0 and 1; a recent work solved multi-valued BA with the same $O(n^2)$ word complexity~\cite{abraham2019asymptotically}.


BA algorithms also differ in the cryptographic assumptions they make and the cryptographic tools they use. Rabin’s coin~\cite{rabin1983randomized} is based on cryptographic secret sharing~\cite{shamir1979share}. Some later works followed suit, and used cryptographic abstractions such as threshold signatures~\cite{abraham2019asymptotically,cachin2005random}. Other works forgo cryptography altogether and instead consider a full information model, where there are no restrictions on the adversary’s computational power~\cite{canetti1993fast,king2013byzantine}. In this model, the problem is harder, and existing works achieve very low resilience~\cite{king2013byzantine} ($n>400f$) or high communication complexity~\cite{canetti1993fast}. In this paper we do use cryptographic primitives. We assume a computationally bounded adversary and rely on the abstraction of a VRF~\cite{micali1999VRF}. VRFs were previously used in blockchain protocols~\cite{Algorand,hanke2018dfinity,Helix} and were also used by Micali~\cite{DBLP:conf/innovations/Micali17} to construct a shared coin in the synchronous model.


Several works~\cite{Abraham2018HotStuffTL,baudet2019state,kwon2014tendermint,naor2019cogsworth,spiegelman2020search} solve BA with subquadratic complexity in the so-called optimistic case (or ``happy path''), when communication is timely and a correct process is chosen as a ``leader''. In contrast, we focus on the worst-case asynchronous case. 


\begin{table}
\caption{Asynchronous Byzantine Agreement algorithms.}

\setlength\extrarowheight{3pt}

\begin{tabular}{lccccc}

\toprule
% \hline
Protocol & n $>$ & Adversary & Word complexity & Termination & Safety \\

\midrule

Ben-Or~\cite{ben1983another}   & $5f$ & adaptive & $O(2^n)$ & w.p. 1 & $\checkmark$ \\ 


Rabin~\cite{rabin1983randomized}   & $10f$ & adaptive & $O(n^2)$ & w.p. 1 & $\checkmark$ \\ 

Bracha~\cite{bracha1987asynchronous} & $3f$  & adaptive & $O(2^n)$ & w.p. 1 & $\checkmark$ \\ 

Cachin et al.~\cite{cachin2005random} & $3f$  & adaptive & $O(n^2)$ &  w.p. 1 & $\checkmark$ \\ 

King-Saia~\cite{king2013byzantine} & $400f$  & adaptive & polynomial & whp & $\checkmark$ \\ 

MMR~\cite{mostefaoui2015signature} & $3f$  & adaptive & $O(n^2)$ & w.p. 1 & $\checkmark$ \\ 

% Section \ref{sec:shared_coin} + MMR & $\approx3.5f$  & delayed-adaptive & $O(n^2)$ & PKI & w.p. 1 & $\checkmark$ \\ 

Our protocol & $\approx4.5f$  & delayed-adaptive & $\tilde{O}(n)$ & whp & whp \\ 

\bottomrule

\end{tabular}
\label{tab:survey}
\end{table}

% \paragraph{Committees.}
{\bf Committees.} 
We use committees in order to reduce the word complexity and allow each step of the protocol to be executed by only a fraction of the processes. King and Saia used a similar concept and presented the first sub-quadratic BA protocol in the synchronous model~\cite{king2011breaking}. Algorand proposed a synchronous algorithm~\cite{Algorand} (and later extended it to eventual synchrony~\cite{chen2018algorand}) where committees are sampled randomly
using a VRF. Each process executes a local computation to sample itself to a committee, and hence the selection of processes does not require interaction among them. We follow this approach in this paper and adapt the technique to the asynchronous model.
 


Following initial publication of our work, Blum et al.~\cite{cryptoeprint:2020:851} have also achieved subquadratic BA WHP under an adaptive adversary. Their assumptions are incomparable to ours -- while they strengthen the adversary to remove the delayed adaptivity requirement, they also strengthen the trusted setup. Specifically, they use a trusted dealer to a priori determine the committee members, flip the shared coin, and share it among the committee members. In contrast, we use a peer-to-peer protocol to generate randomness, and require delayed adaptivity in order to prevent the adversary from tampering with this randomness. As in our protocol, setup has to occur once and may be used for any number of BA instances.
